Swift Ultraviolet Observations of Supernova 2014J in M82: Large Extinction from Interstellar Dust

We present optical and ultraviolet (UV) photometry and spectra of the very nearby and highly reddened supernova (SN) 2014J in M82 obtained with the Swift Ultra-Violet/Optical Telescope (UVOT). Comparison of the UVOT grism spectra of SN~2014J with Hubble Space Telescope observations of SN2011fe or UVOT grism spectra of SN~2012fr are consistent with an extinction law with a low value of R_V~1.4. The high reddening causes the detected photon distribution in the broadband UV filters to have a much longer effective wavelength than for an unreddened SN. The light curve evolution is consistent with this shift and does not show a flattening due to photons being scattered back into the line of sight. The light curve shapes and color evolution are inconsistent with a contribution scattered into the line of sight by circumstellar dust. We conclude that most or all of the high reddening must come from interstellar dust. We show that even for a single dust composition, there is not a unique reddening law caused by circumstellar scattering. Rather, when considering scattering from a time-variable source, we confirm earlier studies that the reddening law is a function of the dust geometry, column density, and epoch. We also show how an assumed geometry of dust as a foreground sheet in mixed stellar/dust systems will lead to a higher inferred R_V. Rather than assuming the dust around SNe is peculiar, SNe may be useful probes of the interstellar reddening laws in other galaxies.

==> tab1.tex <==
SN2014J   & UVW2     & 56679.4377 &  17.050 &   0.088 &  20.095 &  11.091 &   1.355 &   0.110 \\
SN2014J   & UVW2     & 56680.1872 &  16.757 &   0.093 &  19.572 &  11.093 &   1.775 &   0.153 \\
SN2014J   & UVW2     & 56680.5998 &  16.636 &   0.087 &  19.823 &  11.091 &   1.984 &   0.159 \\
SN2014J   & UVW2     & 56681.3990 &  16.431 &   0.084 &  19.810 &  11.091 &   2.396 &   0.185 \\
SN2014J   & UVW2     & 56682.1699 &  16.271 &   0.082 &  19.789 &  11.091 &   2.776 &   0.210 \\
SN2014J   & UVW2     & 56682.6802 &  16.241 &   0.076 &  20.288 &  11.092 &   2.855 &   0.200 \\
SN2014J   & UVW2     & 56683.4062 &  16.108 &   0.080 &  19.810 &  11.091 &   3.227 &   0.238 \\
SN2014J   & UVW2     & 56684.3993 &  15.965 &   0.079 &  19.799 &  11.091 &   3.682 &   0.267 \\
SN2014J   & UVW2     & 56685.6791 &  15.936 &   0.078 &  19.798 &  11.091 &   3.780 &   0.273 \\
SN2014J   & UVW2     & 56686.8127 &  15.868 &   0.078 &  19.793 &  11.091 &   4.027 &   0.289 \\
SN2014J   & UVW2     & 56687.9318 &  15.866 &   0.078 &  19.805 &  11.091 &   4.031 &   0.289 \\
SN2014J   & UVW2     & 56688.3326 &  15.807 &   0.077 &  19.807 &  11.091 &   4.258 &   0.304 \\
SN2014J   & UVW2     & 56689.4154 &  15.840 &   0.075 &  20.126 &  11.092 &   4.129 &   0.284 \\
SN2014J   & UVW2     & 56689.5060 &  15.811 &   0.061 &  21.197 &  11.091 &   4.244 &   0.237 \\
SN2014J   & UVW2     & 56689.3352 &  15.870 &   0.078 &  19.797 &  11.091 &   4.018 &   0.288 \\
SN2014J   & UVW2     & 56690.3322 &  15.811 &   0.077 &  19.803 &  11.091 &   4.242 &   0.303 \\
SN2014J   & UVW2     & 56691.0513 &  15.921 &   0.081 &  19.616 &  11.091 &   3.832 &   0.285 \\
SN2014J   & UVW2     & 56691.1180 &  15.853 &   0.081 &  19.544 &  11.091 &   4.081 &   0.304 \\
SN2014J   & UVW2     & 56691.4652 &  15.875 &   0.078 &  19.801 &  11.091 &   3.998 &   0.287 \\
SN2014J   & UVW2     & 56692.3341 &  15.867 &   0.078 &  19.797 &  11.091 &   4.031 &   0.289 \\
SN2014J   & UVW2     & 56692.7855 &  15.882 &   0.093 &  18.970 &  11.091 &   3.972 &   0.342 \\
SN2014J   & UVW2     & 56693.6643 &  15.941 &   0.079 &  19.798 &  11.091 &   3.763 &   0.272 \\
SN2014J   & UVW2     & 56693.8408 &  15.960 &   0.081 &  19.610 &  11.091 &   3.698 &   0.277 \\
SN2014J   & UVW2     & 56693.9076 &  15.969 &   0.082 &  19.586 &  11.091 &   3.667 &   0.277 \\
SN2014J   & UVW2     & 56695.5312 &  16.077 &   0.080 &  19.815 &  11.091 &   3.319 &   0.244 \\
SN2014J   & UVW2     & 56695.5189 &  16.111 &   0.104 &  18.822 &  11.091 &   3.220 &   0.310 \\
SN2014J   & UVW2     & 56695.6754 &  16.055 &   0.087 &  19.358 &  11.091 &   3.389 &   0.272 \\
SN2014J   & UVW2     & 56696.6653 &  16.068 &   0.080 &  19.801 &  11.091 &   3.348 &   0.246 \\
SN2014J   & UVW2     & 56696.7182 &  16.077 &   0.103 &  18.837 &  11.091 &   3.319 &   0.316 \\
SN2014J   & UVW2     & 56696.8113 &  16.046 &   0.088 &  19.317 &  11.091 &   3.418 &   0.278 \\
SN2014J   & UVW2     & 56697.3344 &  16.142 &   0.080 &  19.808 &  11.091 &   3.126 &   0.231 \\
SN2014J   & UVW2     & 56698.6650 &  16.043 &   0.079 &  19.790 &  11.091 &   3.425 &   0.251 \\
SN2014J   & UVW2     & 56699.2681 &  16.370 &   0.083 &  19.804 &  11.091 &   2.536 &   0.194 \\
SN2014J   & UVW2     & 56701.4638 &  16.549 &   0.085 &  19.801 &  11.091 &   2.149 &   0.169 \\
SN2014J   & UVW2     & 56702.8638 &  16.632 &   0.087 &  19.807 &  11.091 &   1.992 &   0.159 \\
SN2014J   & UVW2     & 56703.7647 &  16.794 &   0.103 &  19.382 &  11.091 &   1.716 &   0.162 \\
SN2014J   & UVW2     & 56705.5305 &  16.859 &   0.091 &  19.795 &  11.092 &   1.615 &   0.135 \\
SN2014J   & UVW2     & 56706.7989 &  17.080 &   0.096 &  19.802 &  11.092 &   1.318 &   0.116 \\
SN2014J   & UVW2     & 56707.7971 &  17.052 &   0.095 &  19.799 &  11.092 &   1.353 &   0.118 \\
SN2014J   & UVW2     & 56708.5978 &  17.123 &   0.097 &  19.794 &  11.092 &   1.267 &   0.113 \\
SN2014J   & UVW2     & 56709.8312 &  17.151 &   0.115 &  19.347 &  11.092 &   1.235 &   0.131 \\
SN2014J   & UVW2     & 56713.0680 &  17.432 &   0.106 &  19.794 &  11.092 &   0.953 &   0.093 \\
SN2014J   & UVW2     & 56749.4827 &  18.773 &   0.192 &  19.814 &  11.091 &   0.277 &   0.049 \\
SN2014J   & UVW2     & 56753.7469 &  18.975 &   0.217 &  19.808 &  11.092 &   0.230 &   0.046 \\
SN2014J   & UVW2     & 56757.4449 &  18.998 &   0.177 &  20.170 &  11.092 &   0.225 &   0.037 \\
SN2014J   & UVM2     & 56679.4496 &    NULL &    NULL &  20.113 &  10.557 &   0.025 &   0.015 \\
SN2014J   & UVM2     & 56680.1989 &    NULL &    NULL &  20.306 &  10.557 &   0.014 &   0.013 \\
SN2014J   & UVM2     & 56680.6036 &    NULL &    NULL &  19.811 &  10.557 &   0.024 &   0.019 \\
SN2014J   & UVM2     & 56681.4042 &  19.999 &   0.249 &  20.549 &  10.557 &   0.055 &   0.013 \\
SN2014J   & UVM2     & 56682.1765 &    NULL &    NULL &  20.125 &  10.557 &   0.034 &   0.016 \\
SN2014J   & UVM2     & 56682.6647 &  20.217 &   0.280 &  20.602 &  10.557 &   0.045 &   0.012 \\
SN2014J   & UVM2     & 56683.4095 &    NULL &    NULL &  19.895 &  10.557 &   0.057 &   0.020 \\
SN2014J   & UVM2     & 56684.4040 &  19.741 &   0.279 &  20.137 &  10.557 &   0.070 &   0.018 \\
SN2014J   & UVM2     & 56684.5704 &  19.790 &   0.145 &  21.147 &  10.557 &   0.067 &   0.009 \\
SN2014J   & UVM2     & 56685.6831 &  19.362 &   0.231 &  20.038 &  10.557 &   0.099 &   0.021 \\
SN2014J   & UVM2     & 56686.4080 &  19.661 &   0.164 &  20.821 &  10.557 &   0.075 &   0.011 \\
SN2014J   & UVM2     & 56686.8159 &  19.921 &   0.351 &  19.995 &  10.557 &   0.059 &   0.019 \\
SN2014J   & UVM2     & 56687.5767 &  19.718 &   0.161 &  20.916 &  10.557 &   0.071 &   0.011 \\
SN2014J   & UVM2     & 56687.9436 &  19.748 &   0.159 &  20.963 &  10.557 &   0.069 &   0.010 \\
SN2014J   & UVM2     & 56688.3363 &  19.137 &   0.230 &  19.838 &  10.557 &   0.122 &   0.026 \\
SN2014J   & UVM2     & 56689.3404 &    NULL &    NULL &  20.205 &  10.557 &   0.040 &   0.015 \\
SN2014J   & UVM2     & 56689.6364 &  19.804 &   0.147 &  21.140 &  10.557 &   0.066 &   0.009 \\
SN2014J   & UVM2     & 56690.3360 &  19.771 &   0.358 &  19.815 &  10.557 &   0.068 &   0.022 \\
SN2014J   & UVM2     & 56690.6795 &  19.808 &   0.148 &  21.131 &  10.557 &   0.066 &   0.009 \\
SN2014J   & UVM2     & 56691.4693 &  19.907 &   0.358 &  19.950 &  10.557 &   0.060 &   0.020 \\
SN2014J   & UVM2     & 56692.3382 &  19.909 &   0.356 &  19.963 &  10.557 &   0.060 &   0.020 \\
SN2014J   & UVM2     & 56692.5330 &  19.762 &   0.141 &  21.171 &  10.557 &   0.068 &   0.009 \\
SN2014J   & UVM2     & 56693.6695 &  19.841 &   0.272 &  20.273 &  10.557 &   0.064 &   0.016 \\
SN2014J   & UVM2     & 56694.9746 &  20.203 &   0.323 &  20.392 &  10.557 &   0.046 &   0.014 \\
SN2014J   & UVM2     & 56695.5363 &  20.018 &   0.313 &  20.250 &  10.557 &   0.054 &   0.016 \\
SN2014J   & UVM2     & 56696.6696 &    NULL &    NULL &  20.026 &  10.557 &   0.047 &   0.018 \\
SN2014J   & UVM2     & 56696.8676 &  20.184 &   0.190 &  21.123 &  10.557 &   0.046 &   0.008 \\
SN2014J   & UVM2     & 56697.3386 &  20.086 &   0.370 &  20.088 &  10.557 &   0.051 &   0.017 \\
SN2014J   & UVM2     & 56698.4636 &  20.730 &   0.272 &  21.176 &  10.557 &   0.028 &   0.007 \\
SN2014J   & UVM2     & 56698.6691 &    NULL &    NULL &  20.145 &  10.557 &   0.045 &   0.016 \\
SN2014J   & UVM2     & 56699.2732 &  20.257 &   0.370 &  20.264 &  10.557 &   0.043 &   0.015 \\
SN2014J   & UVM2     & 56701.4692 &    NULL &    NULL &  20.322 &  10.557 &   0.023 &   0.013 \\
SN2014J   & UVM2     & 56702.4981 &  21.025 &   0.374 &  21.056 &  10.557 &   0.021 &   0.007 \\
SN2014J   & UVM2     & 56702.8689 &    NULL &    NULL &  20.238 &  10.557 &   0.028 &   0.014 \\
SN2014J   & UVM2     & 56703.7683 &    NULL &    NULL &  19.232 &  10.557 &  -0.000 &   0.026 \\
SN2014J   & UVM2     & 56705.5345 &    NULL &    NULL &  20.289 &  10.557 &   0.034 &   0.014 \\
SN2014J   & UVM2     & 56706.2644 &  21.122 &   0.325 &  21.353 &  10.557 &   0.020 &   0.006 \\
SN2014J   & UVM2     & 56706.8050 &    NULL &    NULL &  20.280 &  10.557 &   0.005 &   0.012 \\
SN2014J   & UVM2     & 56707.8015 &    NULL &    NULL &  20.046 &  10.557 &   0.014 &   0.015 \\
SN2014J   & UVM2     & 56708.6017 &    NULL &    NULL &  19.962 &  10.557 &  -0.015 &   0.014 \\
SN2014J   & UVM2     & 56709.8356 &    NULL &    NULL &  19.588 &  10.557 &   0.019 &   0.022 \\
SN2014J   & UVM2     & 56710.4989 &    NULL &    NULL &  21.305 &  10.557 &   0.014 &   0.006 \\
SN2014J   & UVM2     & 56713.0724 &    NULL &    NULL &  19.929 &  10.557 &   0.031 &   0.018 \\
SN2014J   & UVM2     & 56749.9231 &    NULL &    NULL &  20.170 &  10.557 &  -0.011 &   0.012 \\
SN2014J   & UVM2     & 56753.7533 &    NULL &    NULL &  20.609 &  10.557 &   0.006 &   0.010 \\
SN2014J   & UVM2     & 56757.4483 &    NULL &    NULL &  20.020 &  10.557 &   0.014 &   0.016 \\
SN2014J   & UVW1     & 56679.4617 &  15.771 &   0.068 &  19.554 &  11.164 &   4.650 &   0.292 \\
SN2014J   & UVW1     & 56680.2002 &  15.614 &   0.069 &  19.332 &  11.164 &   5.375 &   0.341 \\
SN2014J   & UVW1     & 56680.5954 &  15.532 &   0.072 &  19.045 &  11.164 &   5.799 &   0.383 \\
SN2014J   & UVW1     & 56681.3946 &  15.241 &   0.069 &  19.039 &  11.163 &   7.576 &   0.479 \\
SN2014J   & UVW1     & 56682.1821 &  15.156 &   0.070 &  18.883 &  11.164 &   8.192 &   0.525 \\
SN2014J   & UVW1     & 56683.4018 &  14.948 &   0.066 &  19.022 &  11.163 &   9.925 &   0.605 \\
SN2014J   & UVW1     & 56684.3949 &  14.868 &   0.066 &  19.015 &  11.163 &  10.681 &   0.646 \\
SN2014J   & UVW1     & 56685.6747 &  14.743 &   0.065 &  19.006 &  11.163 &  11.985 &   0.716 \\
SN2014J   & UVW1     & 56686.8083 &  14.616 &   0.060 &  19.004 &  11.163 &  13.476 &   0.748 \\
SN2014J   & UVW1     & 56687.2067 &  14.598 &   0.048 &  20.232 &  11.163 &  13.709 &   0.600 \\
SN2014J   & UVW1     & 56687.7679 &  14.595 &   0.048 &  20.215 &  11.163 &  13.741 &   0.603 \\
SN2014J   & UVW1     & 56687.9604 &  14.569 &   0.057 &  19.223 &  11.163 &  14.070 &   0.735 \\
SN2014J   & UVW1     & 56688.3281 &  14.585 &   0.060 &  19.004 &  11.163 &  13.864 &   0.760 \\
SN2014J   & UVW1     & 56689.3308 &  14.635 &   0.061 &  19.002 &  11.163 &  13.242 &   0.741 \\
SN2014J   & UVW1     & 56690.3278 &  14.662 &   0.061 &  19.003 &  11.163 &  12.915 &   0.731 \\
SN2014J   & UVW1     & 56691.4607 &  14.698 &   0.062 &  19.006 &  11.163 &  12.499 &   0.718 \\
SN2014J   & UVW1     & 56692.3296 &  14.772 &   0.065 &  19.008 &  11.163 &  11.668 &   0.698 \\
SN2014J   & UVW1     & 56693.6599 &  14.858 &   0.066 &  19.016 &  11.163 &  10.784 &   0.651 \\
SN2014J   & UVW1     & 56695.5267 &  14.912 &   0.066 &  18.991 &  11.164 &  10.260 &   0.623 \\
SN2014J   & UVW1     & 56695.6603 &  14.937 &   0.065 &  19.138 &  11.163 &  10.027 &   0.600 \\
SN2014J   & UVW1     & 56696.6609 &  14.999 &   0.067 &  19.022 &  11.163 &   9.474 &   0.580 \\
SN2014J   & UVW1     & 56697.3300 &  15.066 &   0.067 &  19.021 &  11.164 &   8.906 &   0.550 \\
SN2014J   & UVW1     & 56698.6606 &  15.212 &   0.068 &  19.027 &  11.164 &   7.781 &   0.490 \\
SN2014J   & UVW1     & 56699.2637 &  15.294 &   0.069 &  19.026 &  11.164 &   7.217 &   0.460 \\
SN2014J   & UVW1     & 56701.4594 &  15.459 &   0.071 &  18.981 &  11.167 &   6.202 &   0.406 \\
SN2014J   & UVW1     & 56702.8594 &  15.572 &   0.072 &  19.030 &  11.164 &   5.589 &   0.372 \\
SN2014J   & UVW1     & 56703.7603 &  15.634 &   0.082 &  18.629 &  11.164 &   5.277 &   0.399 \\
SN2014J   & UVW1     & 56705.5261 &  15.883 &   0.077 &  19.026 &  11.165 &   4.196 &   0.297 \\
SN2014J   & UVW1     & 56706.7945 &  15.910 &   0.077 &  19.032 &  11.165 &   4.093 &   0.292 \\
SN2014J   & UVW1     & 56707.7927 &  16.037 &   0.080 &  19.014 &  11.166 &   3.642 &   0.268 \\
SN2014J   & UVW1     & 56708.5934 &  16.159 &   0.082 &  19.018 &  11.166 &   3.253 &   0.247 \\
SN2014J   & UVW1     & 56709.8944 &  16.244 &   0.084 &  19.019 &  11.166 &   3.008 &   0.234 \\
SN2014J   & UVW1     & 56713.0635 &  16.510 &   0.092 &  19.020 &  11.166 &   2.354 &   0.199 \\
SN2014J   & UVW1     & 56749.4783 &  18.036 &   0.191 &  19.052 &  11.165 &   0.578 &   0.101 \\
SN2014J   & UVW1     & 56753.7425 &  17.903 &   0.177 &  19.040 &  11.166 &   0.653 &   0.106 \\
SN2014J   & UVW1     & 56757.4404 &  18.346 &   0.190 &  19.402 &  11.166 &   0.434 &   0.076 \\
SN2014J   & U        & 56680.5633 &  13.814 &   0.039 &  17.873 &  11.061 &  64.624 &   2.323 \\
SN2014J   & U        & 56680.6300 &  13.793 &   0.039 &  17.876 &  11.061 &  65.859 &   2.350 \\
SN2014J   & U        & 56681.3625 &  13.650 &   0.037 &  17.863 &  11.061 &  75.172 &   2.572 \\
SN2014J   & U        & 56681.4291 &  13.575 &   0.036 &  17.855 &  11.060 &  80.567 &   2.702 \\
SN2014J   & U        & 56682.0345 &  13.458 &   0.034 &  18.210 &  11.060 &  89.694 &   2.841 \\
SN2014J   & U        & 56683.3758 &  13.257 &   0.034 &  17.808 &  11.059 & 107.927 &   3.369 \\
SN2014J   & U        & 56683.4303 &  13.227 &   0.034 &  17.796 &  11.059 & 110.984 &   3.446 \\
SN2014J   & U        & 56684.3628 &  13.112 &   0.033 &  17.774 &  11.058 & 123.413 &   3.755 \\
SN2014J   & U        & 56684.4295 &  13.147 &   0.033 &  17.783 &  11.058 & 119.462 &   3.656 \\
SN2014J   & U        & 56685.6426 &  13.044 &   0.033 &  17.768 &  11.058 & 131.391 &   3.952 \\
SN2014J   & U        & 56685.7093 &  13.022 &   0.033 &  17.766 &  11.058 & 134.029 &   4.016 \\
SN2014J   & U        & 56686.7748 &  12.988 &   0.032 &  17.756 &  11.057 & 138.264 &   4.123 \\
SN2014J   & U        & 56686.8443 &  12.975 &   0.032 &  17.756 &  11.057 & 139.946 &   4.164 \\
SN2014J   & U        & 56687.8941 &  13.002 &   0.032 &  17.759 &  11.057 & 136.470 &   4.078 \\
SN2014J   & U        & 56687.9631 &  12.976 &   0.032 &  17.749 &  11.057 & 139.780 &   4.162 \\
SN2014J   & U        & 56688.0291 &  12.984 &   0.032 &  17.749 &  11.058 & 138.807 &   4.138 \\
SN2014J   & U        & 56688.2962 &  13.000 &   0.032 &  17.760 &  11.057 & 136.722 &   4.084 \\
SN2014J   & U        & 56688.3626 &  12.986 &   0.032 &  17.773 &  11.057 & 138.486 &   4.125 \\
SN2014J   & U        & 56689.3029 &  13.036 &   0.033 &  17.773 &  11.058 & 132.269 &   3.972 \\
SN2014J   & U        & 56689.3612 &  13.037 &   0.033 &  17.768 &  11.058 & 132.181 &   3.971 \\
SN2014J   & U        & 56690.2956 &  13.060 &   0.033 &  17.773 &  11.058 & 129.379 &   3.902 \\
SN2014J   & U        & 56690.3625 &  13.076 &   0.033 &  17.768 &  11.058 & 127.482 &   3.857 \\
SN2014J   & U        & 56691.4288 &  13.136 &   0.033 &  17.787 &  11.058 & 120.698 &   3.685 \\
SN2014J   & U        & 56691.4952 &  13.141 &   0.033 &  17.791 &  11.058 & 120.065 &   3.668 \\
SN2014J   & U        & 56692.2950 &  13.221 &   0.034 &  17.802 &  11.059 & 111.547 &   3.459 \\
SN2014J   & U        & 56692.3668 &  13.247 &   0.034 &  17.808 &  11.059 & 108.901 &   3.394 \\
SN2014J   & U        & 56693.6278 &  13.319 &   0.034 &  17.820 &  11.059 & 101.910 &   3.221 \\
SN2014J   & U        & 56693.6945 &  13.298 &   0.034 &  17.816 &  11.059 & 103.931 &   3.272 \\
SN2014J   & U        & 56695.4947 &  13.481 &   0.036 &  17.842 &  11.060 &  87.841 &   2.877 \\
SN2014J   & U        & 56695.5613 &  13.482 &   0.036 &  17.842 &  11.060 &  87.704 &   2.874 \\
SN2014J   & U        & 56696.6288 &  13.567 &   0.036 &  17.843 &  11.060 &  81.145 &   2.718 \\
SN2014J   & U        & 56696.6955 &  13.560 &   0.036 &  17.842 &  11.060 &  81.668 &   2.731 \\
SN2014J   & U        & 56697.2979 &  13.687 &   0.038 &  17.863 &  11.061 &  72.652 &   2.513 \\
SN2014J   & U        & 56697.3646 &  13.661 &   0.037 &  17.860 &  11.061 &  74.383 &   2.554 \\
SN2014J   & U        & 56698.6297 &  13.781 &   0.039 &  17.875 &  11.061 &  66.598 &   2.369 \\
SN2014J   & U        & 56698.6940 &  13.801 &   0.039 &  17.880 &  11.062 &  65.380 &   2.340 \\
SN2014J   & U        & 56699.2359 &  13.887 &   0.040 &  17.884 &  11.062 &  60.402 &   2.223 \\
SN2014J   & U        & 56699.2940 &  13.859 &   0.040 &  17.887 &  11.062 &  61.998 &   2.259 \\
SN2014J   & U        & 56701.4273 &  14.049 &   0.042 &  17.902 &  11.062 &  52.031 &   2.026 \\
SN2014J   & U        & 56701.4940 &  14.078 &   0.043 &  17.904 &  11.062 &  50.685 &   1.996 \\
SN2014J   & U        & 56702.8273 &  14.244 &   0.046 &  17.913 &  11.063 &  43.507 &   1.833 \\
SN2014J   & U        & 56702.8940 &  14.242 &   0.046 &  17.914 &  11.063 &  43.574 &   1.834 \\
SN2014J   & U        & 56703.7615 &  14.425 &   0.050 &  17.925 &  11.063 &  36.818 &   1.680 \\
SN2014J   & U        & 56705.4940 &  14.606 &   0.054 &  17.938 &  11.064 &  31.155 &   1.555 \\
SN2014J   & U        & 56705.5606 &  14.624 &   0.055 &  17.934 &  11.064 &  30.660 &   1.547 \\
SN2014J   & U        & 56706.7642 &  14.744 &   0.058 &  17.941 &  11.064 &  27.433 &   1.474 \\
SN2014J   & U        & 56706.8273 &  14.759 &   0.059 &  17.930 &  11.065 &  27.063 &   1.474 \\
SN2014J   & U        & 56707.7606 &  14.914 &   0.065 &  17.933 &  11.066 &  23.471 &   1.398 \\
SN2014J   & U        & 56707.8273 &  14.917 &   0.065 &  17.918 &  11.067 &  23.410 &   1.405 \\
SN2014J   & U        & 56708.5613 &  15.102 &   0.072 &  17.940 &  11.066 &  19.736 &   1.317 \\
SN2014J   & U        & 56708.6280 &  15.050 &   0.070 &  17.929 &  11.066 &  20.710 &   1.343 \\
SN2014J   & U        & 56709.8280 &  15.344 &   0.083 &  17.931 &  11.067 &  15.790 &   1.201 \\
SN2014J   & U        & 56709.9634 &  15.166 &   0.078 &  17.948 &  11.065 &  18.605 &   1.331 \\
SN2014J   & U        & 56713.0315 &  15.590 &   0.090 &  17.950 &  11.066 &  12.589 &   1.049 \\
SN2014J   & U        & 56713.0981 &  15.699 &   0.095 &  17.952 &  11.066 &  11.392 &   0.992 \\
SN2014J   & U        & 56723.3938 &  16.263 &   0.096 &  18.449 &  11.065 &   6.772 &   0.601 \\
SN2014J   & U        & 56727.5881 &  16.544 &   0.110 &  18.435 &  11.065 &   5.229 &   0.532 \\
SN2014J   & U        & 56731.0566 &  16.635 &   0.116 &  18.450 &  11.065 &   4.810 &   0.514 \\
SN2014J   & U        & 56731.4032 &  16.667 &   0.118 &  18.457 &  11.065 &   4.670 &   0.508 \\
SN2014J   & U        & 56731.5839 &  16.589 &   0.113 &  18.447 &  11.065 &   5.019 &   0.523 \\
SN2014J   & U        & 56735.2484 &  16.673 &   0.118 &  18.447 &  11.065 &   4.645 &   0.507 \\
SN2014J   & U        & 56739.6554 &  16.643 &   0.117 &  18.458 &  11.065 &   4.775 &   0.513 \\
SN2014J   & U        & 56743.7220 &  16.916 &   0.136 &  18.457 &  11.065 &   3.713 &   0.465 \\
SN2014J   & U        & 56749.0464 &  16.814 &   0.169 &  17.964 &  11.066 &   4.079 &   0.636 \\
SN2014J   & U        & 56749.9128 &  16.775 &   0.165 &  17.962 &  11.066 &   4.228 &   0.644 \\
SN2014J   & U        & 56753.7113 &  16.939 &   0.185 &  17.949 &  11.069 &   3.634 &   0.619 \\
SN2014J   & U        & 56753.7761 &  17.070 &   0.205 &  17.916 &  11.072 &   3.220 &   0.609 \\
SN2014J   & U        & 56757.0417 &  16.872 &   0.181 &  17.903 &  11.073 &   3.867 &   0.645 \\
SN2014J   & U        & 56757.4412 &  16.775 &   0.170 &  17.914 &  11.072 &   4.228 &   0.661 \\
SN2014J   & U        & 56757.5134 &  16.925 &   0.182 &  17.962 &  11.067 &   3.682 &   0.618 \\
SN2014J   & U        & 56757.8417 &  17.042 &   0.204 &  17.895 &  11.074 &   3.305 &   0.621 \\
SN2014J   & B        & 56680.5646 &  12.746 &   0.031 &  17.478 &  11.872 & 351.173 &  10.186 \\
SN2014J   & B        & 56680.6313 &  12.785 &   0.032 &  17.495 &  11.873 & 338.915 &   9.873 \\
SN2014J   & B        & 56681.3638 &  12.592 &   0.031 &  17.407 &  11.867 & 404.637 &  11.554 \\
SN2014J   & B        & 56681.4304 &  12.600 &   0.031 &  17.411 &  11.867 & 401.944 &  11.487 \\
SN2014J   & B        & 56682.0362 &  12.513 &   0.031 &  17.610 &  11.865 & 435.367 &  12.318 \\
SN2014J   & B        & 56683.3771 &  12.373 &   0.030 &  17.293 &  11.859 & 495.171 &  13.879 \\
SN2014J   & B        & 56683.4316 &  12.323 &   0.030 &  17.261 &  11.858 & 518.411 &  14.482 \\
SN2014J   & B        & 56684.3641 &  12.243 &   0.030 &  17.211 &  11.855 & 557.971 &  15.498 \\
SN2014J   & B        & 56684.4307 &  12.233 &   0.030 &  17.204 &  11.855 & 563.129 &  15.634 \\
SN2014J   & B        & 56685.6439 &  12.156 &   0.030 &  17.161 &  11.852 & 604.767 &  16.703 \\
SN2014J   & B        & 56685.7105 &  12.141 &   0.030 &  17.151 &  11.851 & 613.191 &  16.922 \\
SN2014J   & B        & 56686.7761 &  12.146 &   0.030 &  17.154 &  11.851 & 610.245 &  16.846 \\
SN2014J   & B        & 56686.8455 &  12.094 &   0.030 &  17.122 &  11.850 & 640.054 &  17.615 \\
SN2014J   & B        & 56687.8954 &  12.052 &   0.030 &  17.084 &  11.848 & 665.721 &  18.282 \\
SN2014J   & B        & 56687.9644 &  12.056 &   0.030 &  17.085 &  11.849 & 663.096 &  18.214 \\
SN2014J   & B        & 56688.2974 &  12.015 &   0.030 &  17.057 &  11.847 & 688.419 &  18.872 \\
SN2014J   & B        & 56688.3639 &  12.065 &   0.030 &  17.110 &  11.849 & 657.523 &  18.065 \\
SN2014J   & B        & 56689.3042 &  12.059 &   0.030 &  17.095 &  11.849 & 661.220 &  18.165 \\
SN2014J   & B        & 56689.3625 &  12.062 &   0.030 &  17.095 &  11.849 & 659.570 &  18.123 \\
SN2014J   & B        & 56690.2969 &  12.081 &   0.030 &  17.111 &  11.849 & 648.287 &  17.830 \\
SN2014J   & B        & 56690.3637 &  12.064 &   0.030 &  17.096 &  11.849 & 658.098 &  18.083 \\
SN2014J   & B        & 56691.4301 &  12.071 &   0.030 &  17.098 &  11.849 & 654.074 &  17.984 \\
SN2014J   & B        & 56691.4964 &  12.073 &   0.030 &  17.106 &  11.849 & 652.681 &  17.943 \\
SN2014J   & B        & 56692.2962 &  12.118 &   0.030 &  17.134 &  11.851 & 626.278 &  17.261 \\
SN2014J   & B        & 56692.3680 &  12.106 &   0.030 &  17.130 &  11.850 & 633.502 &  17.445 \\
SN2014J   & B        & 56693.6291 &  12.089 &   0.030 &  17.114 &  11.850 & 643.391 &  17.705 \\
SN2014J   & B        & 56693.6958 &  12.143 &   0.030 &  17.151 &  11.852 & 612.187 &  16.900 \\
SN2014J   & B        & 56695.4959 &  12.188 &   0.030 &  17.177 &  11.853 & 587.473 &  16.260 \\
SN2014J   & B        & 56695.5626 &  12.188 &   0.030 &  17.176 &  11.853 & 587.305 &  16.258 \\
SN2014J   & B        & 56696.6300 &  12.215 &   0.030 &  17.189 &  11.854 & 572.919 &  15.884 \\
SN2014J   & B        & 56696.6968 &  12.300 &   0.030 &  17.245 &  11.857 & 529.747 &  14.775 \\
SN2014J   & B        & 56697.2992 &  12.319 &   0.030 &  17.254 &  11.858 & 520.679 &  14.543 \\
SN2014J   & B        & 56697.3658 &  12.294 &   0.030 &  17.241 &  11.857 & 532.573 &  14.846 \\
SN2014J   & B        & 56698.6310 &  12.381 &   0.030 &  17.293 &  11.860 & 491.692 &  13.792 \\
SN2014J   & B        & 56698.6952 &  12.374 &   0.030 &  17.291 &  11.860 & 494.571 &  13.870 \\
SN2014J   & B        & 56699.2372 &  12.451 &   0.031 &  17.335 &  11.862 & 460.865 &  12.995 \\
SN2014J   & B        & 56699.2952 &  12.460 &   0.031 &  17.339 &  11.863 & 456.878 &  12.898 \\
SN2014J   & B        & 56701.4285 &  12.610 &   0.031 &  17.413 &  11.868 & 398.105 &  11.392 \\
SN2014J   & B        & 56701.4952 &  12.595 &   0.031 &  17.408 &  11.867 & 403.775 &  11.533 \\
SN2014J   & B        & 56702.8286 &  12.732 &   0.031 &  17.471 &  11.872 & 355.699 &  10.304 \\
SN2014J   & B        & 56702.8953 &  12.698 &   0.031 &  17.456 &  11.871 & 367.049 &  10.595 \\
SN2014J   & B        & 56703.7628 &  12.822 &   0.032 &  17.506 &  11.875 & 327.617 &   9.587 \\
SN2014J   & B        & 56705.4952 &  12.961 &   0.032 &  17.565 &  11.879 & 288.259 &   8.585 \\
SN2014J   & B        & 56705.5619 &  12.985 &   0.032 &  17.571 &  11.880 & 281.724 &   8.425 \\
SN2014J   & B        & 56706.7654 &  13.146 &   0.033 &  17.632 &  11.884 & 243.078 &   7.438 \\
SN2014J   & B        & 56706.8286 &  13.126 &   0.033 &  17.621 &  11.884 & 247.566 &   7.558 \\
SN2014J   & B        & 56707.7619 &  13.191 &   0.034 &  17.640 &  11.887 & 233.109 &   7.196 \\
SN2014J   & B        & 56707.8285 &  13.216 &   0.034 &  17.646 &  11.888 & 227.843 &   7.067 \\
SN2014J   & B        & 56708.5626 &  13.320 &   0.034 &  17.679 &  11.890 & 206.944 &   6.536 \\
SN2014J   & B        & 56708.6292 &  13.281 &   0.034 &  17.664 &  11.890 & 214.547 &   6.736 \\
SN2014J   & B        & 56709.8293 &  13.414 &   0.035 &  17.699 &  11.893 & 189.839 &   6.120 \\
SN2014J   & B        & 56709.9646 &  13.408 &   0.035 &  17.704 &  11.892 & 190.836 &   6.130 \\
SN2014J   & B        & 56713.0327 &  13.721 &   0.038 &  17.775 &  11.900 & 143.034 &   4.954 \\
SN2014J   & B        & 56713.0994 &  13.718 &   0.038 &  17.776 &  11.899 & 143.448 &   4.961 \\
SN2014J   & B        & 56723.3958 &  14.504 &   0.048 &  18.201 &  11.911 &  69.594 &   3.103 \\
SN2014J   & B        & 56727.5901 &  14.802 &   0.058 &  18.209 &  11.913 &  52.850 &   2.827 \\
SN2014J   & B        & 56731.0585 &  14.864 &   0.059 &  18.214 &  11.913 &  49.936 &   2.709 \\
SN2014J   & B        & 56731.4052 &  14.894 &   0.060 &  18.219 &  11.914 &  48.584 &   2.663 \\
SN2014J   & B        & 56731.5859 &  14.897 &   0.059 &  18.219 &  11.913 &  48.422 &   2.650 \\
SN2014J   & B        & 56735.2504 &  14.897 &   0.059 &  18.223 &  11.914 &  48.437 &   2.649 \\
SN2014J   & B        & 56739.6573 &  14.982 &   0.061 &  18.233 &  11.914 &  44.779 &   2.506 \\
SN2014J   & B        & 56743.7240 &  15.034 &   0.061 &  18.228 &  11.914 &  42.681 &   2.415 \\
SN2014J   & B        & 56749.0476 &  15.212 &   0.073 &  17.929 &  11.917 &  36.237 &   2.421 \\
SN2014J   & B        & 56749.9140 &  15.077 &   0.069 &  17.914 &  11.916 &  41.057 &   2.621 \\
SN2014J   & B        & 56753.7126 &  15.093 &   0.070 &  17.915 &  11.918 &  40.450 &   2.593 \\
SN2014J   & B        & 56753.7774 &  15.002 &   0.068 &  17.894 &  11.923 &  43.970 &   2.742 \\
SN2014J   & B        & 56757.0430 &  15.132 &   0.071 &  17.896 &  11.928 &  39.025 &   2.544 \\
SN2014J   & B        & 56757.4424 &  15.104 &   0.070 &  17.895 &  11.926 &  40.044 &   2.587 \\
SN2014J   & B        & 56757.5146 &  15.014 &   0.068 &  17.916 &  11.916 &  43.504 &   2.716 \\
SN2014J   & B        & 56757.8430 &  15.140 &   0.071 &  17.889 &  11.928 &  38.725 &   2.534 \\
SN2014J   & V        & 56680.5682 &  11.529 &   0.031 &  16.303 &  10.645 & 350.296 &  10.058 \\
SN2014J   & V        & 56680.6349 &  11.528 &   0.031 &  16.303 &  10.645 & 350.525 &  10.064 \\
SN2014J   & V        & 56681.3674 &  11.397 &   0.031 &  16.248 &  10.641 & 395.478 &  11.215 \\
SN2014J   & V        & 56681.4340 &  11.403 &   0.031 &  16.251 &  10.641 & 393.399 &  11.162 \\
SN2014J   & V        & 56682.0396 &  11.277 &   0.030 &  16.438 &  10.638 & 441.834 &  12.376 \\
SN2014J   & V        & 56683.3807 &  11.139 &   0.030 &  16.115 &  10.633 & 501.765 &  13.948 \\
SN2014J   & V        & 56683.4352 &  11.147 &   0.030 &  16.116 &  10.634 & 497.921 &  13.849 \\
SN2014J   & V        & 56684.3677 &  11.005 &   0.030 &  16.032 &  10.629 & 567.418 &  15.642 \\
SN2014J   & V        & 56684.4344 &  11.040 &   0.030 &  16.054 &  10.630 & 549.463 &  15.177 \\
SN2014J   & V        & 56685.6475 &  10.921 &   0.030 &  15.988 &  10.627 & 613.141 &  16.817 \\
SN2014J   & V        & 56685.7142 &  10.903 &   0.030 &  15.975 &  10.626 & 623.609 &  17.089 \\
SN2014J   & V        & 56686.7797 &  10.872 &   0.030 &  15.953 &  10.625 & 641.293 &  17.546 \\
SN2014J   & V        & 56686.8492 &  10.850 &   0.030 &  15.939 &  10.625 & 654.846 &  17.899 \\
SN2014J   & V        & 56687.8990 &  10.802 &   0.030 &  15.903 &  10.623 & 684.288 &  18.660 \\
SN2014J   & V        & 56687.9680 &  10.781 &   0.030 &  15.887 &  10.622 & 697.348 &  18.997 \\
SN2014J   & V        & 56688.3011 &  10.765 &   0.030 &  15.876 &  10.622 & 707.997 &  19.276 \\
SN2014J   & V        & 56688.3675 &  10.804 &   0.030 &  15.920 &  10.623 & 683.149 &  18.625 \\
SN2014J   & V        & 56689.3078 &  10.795 &   0.030 &  15.903 &  10.623 & 688.661 &  18.772 \\
SN2014J   & V        & 56689.3661 &  10.797 &   0.030 &  15.903 &  10.623 & 687.595 &  18.745 \\
SN2014J   & V        & 56690.3005 &  10.769 &   0.030 &  15.887 &  10.622 & 705.502 &  19.204 \\
SN2014J   & V        & 56690.3674 &  10.772 &   0.030 &  15.883 &  10.622 & 703.550 &  19.157 \\
SN2014J   & V        & 56691.4337 &  10.744 &   0.030 &  15.863 &  10.621 & 722.046 &  19.637 \\
SN2014J   & V        & 56691.5000 &  10.764 &   0.030 &  15.882 &  10.622 & 708.886 &  19.294 \\
SN2014J   & V        & 56692.2999 &  10.722 &   0.029 &  15.851 &  10.620 & 736.863 &  20.017 \\
SN2014J   & V        & 56692.3717 &  10.749 &   0.030 &  15.873 &  10.621 & 718.424 &  19.541 \\
SN2014J   & V        & 56693.6327 &  10.730 &   0.030 &  15.858 &  10.621 & 730.891 &  19.862 \\
SN2014J   & V        & 56693.6994 &  10.803 &   0.030 &  15.910 &  10.623 & 683.706 &  18.642 \\
SN2014J   & V        & 56695.4996 &  10.775 &   0.030 &  15.886 &  10.622 & 701.340 &  19.102 \\
SN2014J   & V        & 56695.5662 &  10.775 &   0.030 &  15.885 &  10.622 & 701.468 &  19.106 \\
SN2014J   & V        & 56696.6337 &  10.797 &   0.030 &  15.899 &  10.623 & 687.160 &  18.735 \\
SN2014J   & V        & 56696.7004 &  10.815 &   0.030 &  15.912 &  10.624 & 675.852 &  18.443 \\
SN2014J   & V        & 56697.3028 &  10.816 &   0.030 &  15.911 &  10.624 & 675.438 &  18.435 \\
SN2014J   & V        & 56697.3695 &  10.829 &   0.030 &  15.921 &  10.624 & 667.518 &  18.226 \\
SN2014J   & V        & 56698.6346 &  10.930 &   0.030 &  15.989 &  10.627 & 608.224 &  16.693 \\
SN2014J   & V        & 56698.6988 &  10.884 &   0.030 &  15.964 &  10.625 & 634.674 &  17.376 \\
SN2014J   & V        & 56699.2408 &  10.904 &   0.030 &  15.974 &  10.626 & 622.735 &  17.067 \\
SN2014J   & V        & 56699.2989 &  10.928 &   0.030 &  15.992 &  10.627 & 609.151 &  16.715 \\
SN2014J   & V        & 56701.4322 &  11.052 &   0.030 &  16.065 &  10.631 & 543.653 &  15.028 \\
SN2014J   & V        & 56701.4988 &  11.042 &   0.030 &  16.060 &  10.630 & 548.403 &  15.149 \\
SN2014J   & V        & 56702.8322 &  11.123 &   0.030 &  16.106 &  10.633 & 509.244 &  14.141 \\
SN2014J   & V        & 56702.8989 &  11.116 &   0.030 &  16.103 &  10.633 & 512.215 &  14.217 \\
SN2014J   & V        & 56703.7664 &  11.163 &   0.030 &  16.125 &  10.634 & 490.526 &  13.659 \\
SN2014J   & V        & 56705.4989 &  11.265 &   0.030 &  16.183 &  10.637 & 446.808 &  12.535 \\
SN2014J   & V        & 56705.5655 &  11.290 &   0.031 &  16.197 &  10.638 & 436.463 &  12.266 \\
SN2014J   & V        & 56706.7691 &  11.332 &   0.031 &  16.218 &  10.639 & 419.819 &  11.838 \\
SN2014J   & V        & 56706.8322 &  11.336 &   0.031 &  16.220 &  10.639 & 418.234 &  11.796 \\
SN2014J   & V        & 56707.7655 &  11.352 &   0.031 &  16.226 &  10.640 & 412.338 &  11.647 \\
SN2014J   & V        & 56707.8322 &  11.370 &   0.031 &  16.234 &  10.640 & 405.673 &  11.477 \\
SN2014J   & V        & 56708.5662 &  11.414 &   0.031 &  16.254 &  10.642 & 389.265 &  11.056 \\
SN2014J   & V        & 56708.6329 &  11.415 &   0.031 &  16.256 &  10.642 & 388.971 &  11.047 \\
SN2014J   & V        & 56709.8329 &  11.475 &   0.031 &  16.282 &  10.643 & 368.124 &  10.513 \\
SN2014J   & V        & 56713.0364 &  11.564 &   0.031 &  16.321 &  10.646 & 339.193 &   9.775 \\
SN2014J   & V        & 56713.1030 &  11.589 &   0.031 &  16.332 &  10.647 & 331.302 &   9.571 \\
SN2014J   & V        & 56723.4014 &  12.109 &   0.033 &  17.104 &  10.660 & 205.394 &   6.243 \\
SN2014J   & V        & 56727.5936 &  12.323 &   0.034 &  17.093 &  10.665 & 168.630 &   5.331 \\
SN2014J   & V        & 56731.0626 &  12.439 &   0.035 &  17.147 &  10.667 & 151.520 &   4.889 \\
SN2014J   & V        & 56731.4071 &  12.474 &   0.036 &  16.887 &  10.667 & 146.683 &   4.843 \\
SN2014J   & V        & 56731.5888 &  12.468 &   0.035 &  17.087 &  10.667 & 147.557 &   4.809 \\
SN2014J   & V        & 56735.2578 &  12.582 &   0.036 &  17.225 &  10.669 & 132.754 &   4.396 \\
SN2014J   & V        & 56739.6651 &  12.712 &   0.037 &  17.258 &  10.671 & 117.827 &   4.021 \\
SN2014J   & V        & 56743.7272 &  12.830 &   0.039 &  17.180 &  10.673 & 105.723 &   3.764 \\
SN2014J   & V        & 56749.0511 &  12.927 &   0.043 &  16.250 &  10.674 &  96.633 &   3.834 \\
SN2014J   & V        & 56749.9176 &  12.984 &   0.042 &  16.668 &  10.675 &  91.690 &   3.584 \\
SN2014J   & V        & 56753.7162 &  13.036 &   0.043 &  16.677 &  10.676 &  87.398 &   3.483 \\
SN2014J   & V        & 56753.7810 &  13.074 &   0.044 &  16.679 &  10.677 &  84.434 &   3.417 \\
SN2014J   & V        & 56757.0466 &  13.232 &   0.047 &  16.693 &  10.679 &  72.993 &   3.158 \\
SN2014J   & V        & 56757.4461 &  13.175 &   0.046 &  16.688 &  10.679 &  76.931 &   3.253 \\
SN2014J   & V        & 56757.8466 &  13.159 &   0.046 &  16.685 &  10.679 &  78.026 &   3.274 \\

